DeepSketch: A New Machine Learning-Based Reference Search Technique for Post-Deduplication Delta Compression

Data reduction in storage systems is becoming increasingly important as an effective solution to minimize the management cost of a data center. To maximize data-reduction efficiency, existing post-deduplication delta-compression techniques perform delta compression along with traditional data deduplication and lossless compression. Unfortunately, we observe that existing techniques achieve significantly lower data-reduction ratios than the optimal due to their limited accuracy in identifying similar data blocks. In this paper, we propose DeepSketch, a new reference search technique for post-deduplication delta compression that leverages the learning-to-hash method to achieve higher accuracy in reference search for delta compression, thereby improving data-reduction efficiency. DeepSketch uses a deep neural network to extract a data block's sketch, i.e., to create an approximate data signature of the block that can preserve similarity with other blocks. Our evaluation using eleven real-world workloads shows that DeepSketch improves the data-reduction ratio by up to 33% (21% on average) over a state-of-the-art post-deduplication delta-compression technique.

==> sections/backups/05_evaluation_with_multiple_candidates.tex <==
\vspace{-1em}
\section{Evaluation\label{sec:evaluation}}
\vspace{-.5em}
In this section, we evaluate the data-reduction benefits and performance/memory overheads compared to the state-of-the-art super feature (SF)-based sketching technique~\cite{zhang-fast-2019}.
%We present experimental results on \prop.  
%We particularly seek to answer the following questions: 
%1) How much does \prop improve the data-reduction ratio compared to state-of-the-art super feature (SF)-based sketching techniques?\js{;} 
%2) Does \prop work efficiently over data sets which are not used for NN training?\js{;} 
%3) Does it achieve reasonable system throughput?

\vspace{-1em}
\subsection{Methodology\label{subsec:methodology}}
\vspace{-.5em}
\head{Evaluation Platform}
We develop a post-deduplication delta-compression platform that is used as a general workbench to implement and evaluate various reference search techniques.\footnote{We plan to open source our platform including the block I/O traces used in our evaluation.}
%We develop a post-deduplication delta compression platform which is used as a general workbench for implementing and evaluating various reference search techniques.
Our platform runs on a server machine that employs Intel's Xeon 4110 CPU with 8 cores running at 2.1~GHz, 128-GB DDR4 DRAM, and 8 Samsung 860PRO 1-TB SSDs, 
while using GeForce RTX 2080 for DNN inference in \prop.
%Our platform runs on a server machine that employs Intel's Xeon 4110 CPU with 8 cores running at 2.1~GHz, 128-GB DDR4 DRAM, and 8 Samsung 860PRO 1-TB SSDs.
%GeForce RTX 2080 is used as a GPU accelerator for DNN training and inference.

Our platform operates as described in \fig{\ref{fig:baseline}}.  
For every host write, it performs deduplication, delta compression, and lossless compression in order.  
It maintains three main data structures: 1) a fingerprint store for deduplication, 2) a sketch store for delta compression, and 3) a reference table for serving future read requests.
The data block size is set to 4 KiB that is identical to the default block size of widely-used file systems~\cite{mathur-linux-2007, custer-microsoft-1994}.
%A unit size of a data block is set to 4 KiB, which is identical to the default block size of widely-used file systems (\eg~ext4~\cite{mathur-linux-2007} and NTFS~\cite{custer-microsoft-1994}).
We use the MD5 cryptographic hash algorithm~\cite{rivest-1992} to generate a 128-bit fingerprint of an incoming data block and the Xdelta delta compression algorithm~\cite{macdonald-phdthesis-2000, macdonald-xdelta} to compress a non-deduplicated data block with its reference block.  
If there are multiple reference blocks similar to an incoming data block, our platform in the default settings uses the first found one as a reference.\footnote{We also evaluate the impact of considering multiple reference candidates on the data reduction ratio of each technique in \sect{\ref{subsec:multi}}.}  
When the platform cannot find a reference block, it compresses the incoming block using the LZ4 algorithm~\cite{collet-lz4}.
We set the threshold for the number of buffered sketches to invoke ANN updates to 128, which we empirically determine to minimize the performance overhead of exhaustive search and prevent too frequent ANN updates.

%\head{Compared Reference Search Techniques}
\head{Baseline Technique}%JS: or Compared Technique?
We compare \prop against \js{\emph{Finesse}~\cite{zhang-fast-2019},} the state-of-the-art SF-based technique \js{that provides much higher throughput while retraining almost the same data-reduction ratio compared to the representative post-deduplication delta compression technique~\cite{shilane-fast-2012}}.
%As explained in \sect{\ref{subsec:motiv_lsh}}, the effectiveness of a SF-based technique highly depends on parameter settings and matching criteria.
We configure Finesse using the default settings presented in~\cite{zhang-fast-2019}, which are already optimized and have been shown to provide the best data-reduction efficiency with low overhead for a wide range of workloads.
%Need to double check
Finesse generates three 192-bit SFs, each of which can be obtained by transposing four features from different hash functions (\ie~twelve (= 3 $\times$ 4) hash functions are used in total). 
It considers that two data blocks are similar if they have one or more matching SFs, and selects the data block that has the largest number of matching SFs with the incoming block as the reference block for delta compression.
%Finesse considers that two data blocks are similar if the two blocks have one or more matching SFs, and selects the data block that has the largest number of matching SFs with the incoming block as the reference block for delta compression.

\head{Workloads}
We use \fix{eleven} block I/O traces collected from real systems.
\tab{\ref{tab:workloads}} summarizes the characteristics of the traces in terms of the size, deduplication ratio (\ie~\emph{Orignial Data-Set Size / Data-Set Size after Deduplication}), and average compression ratio (\ie~\emph{Original Data-Set Size / Compressed Data-Set Size}).
We collect the I/O traces including contents written in the storage system from real desktop machines and servers while running different applications.
%We collect the I/O traces including contents written in the storage system by tracing every block I/O request in real desktop machines and servers while running different applications.  

\begin{table}[!h]
	\centering
	\vspace{-.5em}
	\caption{Summary of the evaluated workloads.}
	\vspace{-1em}
	\resizebox{1\columnwidth}{!}{%
	\begin{tabular}{ccccc}
		\toprule
		\multirow{2}{*}{\textbf{Workload}} & \multirow{2}{*}{\textbf{Description}} & \multirow{2}{*}{\textbf{Size}} & \textbf{Dedup.} & \textbf{Comp.} \\
		& & & \textbf{ratio} & \textbf{ratio} \\
		\midrule
		%\textbf{\textsf{PC0}} & {General Ubuntu PC usage} & 920 MB & 1.504 & 2.849 \\
		%\hhline{-~---}
		\textbf{\textsf{PC}} & General Ubuntu PC usage & 1.57 GB & 1.381 & 2.209 \\
		\hline
		\textbf{\textsf{Install}} & Installing \& executing programs & 8.83 GB & 1.309 & 2.45 \\
		\hline
		\textbf{\textsf{Update}} & Updating \& downloading SW packages & 3.73 GB & 1.249 & 2.116 \\
		\hline
		\textbf{\textsf{Synth}} & Synthesizing hardware modules & 653 MB & 1.898 & 2.083 \\
		\hline
		\textbf{\textsf{Sensor}} & Sensor data in semiconductor fabrication &  91.2 MB & 1.269 & 12.38 \\
		\hline
		\textbf{\textsf{Web}} & Web page caching & 959 MB & 1.9 & 6.84\\
		\hline
		\textbf{\textsf{SOF0}} &  & 8.98 GB & 1.007 & 2.088\\
		\hhline{-~---}
		\textbf{\textsf{SOF1}} & Storing Stack Overflow database~\cite{sof} & 13.6 GB & 1.01 & 1.997 \\
		\hhline{-~---}
		\textbf{\textsf{SOF2}} & as of 2010 (\sof{0}) and 2013 (\sof{1--4}) & 13.6 GB & 1.01 & 1.996 \\
		\hhline{-~---}
		\textbf{\textsf{SOF3}} &  & 13.6 GB & 1.01 & 1.997 \\
		\hhline{-~---}
		\textbf{\textsf{SOF4}} &  & 13.6 GB & 1.01 & 1.996 \\
		\bottomrule
	\end{tabular}}
	\label{tab:workloads}%
	\vspace{-.5em}
\end{table}%

For \prop, we use different sets of data for training and testing.
In order to evaluate the \emph{adaptability} of \prop (\ie~how well \prop operates under a workload totally different from ones used in its DNN training), we do \emph{not} use the five traces collected from Stack Overflow database~\cite{sof} (\sof{0--4}) for training the DNN of \prop.
%First, in order to evaluate the \emph{adaptability} of \prop (\ie~how well \prop operates under a workload totally different from ones used in its DNN training), we do \emph{not} use the five traces collected from Stack Overflow database~\cite{sof} (\sof{0--4}) for training the DNN of \prop.
By default, we train \prop's DNN model using 10\% of all the remaining six traces and evaluate \prop with the remaining 90\% of each trace\footnote{We also evaluate the impact of the training data-set size in \sect{\ref{subsec:tdata}}.}.
%For the remaining six traces, we use 10\% of each trace for training a DNN model and the remaining 90\% to evaluate \prop on data reduction.  

\begin{figure}[!b]
    \centering
    \vspace{-1em}
    \includegraphics[width=\linewidth]{figs/r_overall_cr.pdf}
    \vspace{-2em}
    \caption{Comparison of overall data-reduction ratio.}
    \label{fig:overall}
\end{figure}

\vspace{-1em}
\subsection{Overall Data Reduction\label{subsec:overall}} 
\vspace{-.5em}
\fig{\ref{fig:overall}} shows the data-reduction ratio after post-dedup\-lication delta compression with the two reference search techniques, Finesse and \prop, under the \fix{eleven} workloads.
%\fig{\ref{fig:overall}} shows the data-reduction ratio (\ie~\emph{Original data-set size / Reduced data-set size}) after post-deduplication delta compression with the two reference search techniques, Finesse and \prop, under the \fix{eleven} workloads.
We only present \sof{1} as a representative result of \sof{1-4} as they show little variations lower than 0.01\%.
%We only present \sof{1} as a representative result of \sof{1-4} as the four workloads show almost the same results with little variations lower than 0.01\%.
All values are normalized to the data-reduction ratios of a baseline system that performs only deduplication and lossless compression in order, which we call \emph{no delta compression (noDC)}.  
%Recall that we obtain the results in \fig{\ref{fig:overall}} using the same DNN model for \prop that is trained with 10\% of each workload, \emph{excluding} the five \sof{} workloads.

We make \js{two} main observations from \fig{\ref{fig:overall}}.  
%First, both Finesse and DeepSketch significantly outperform noDC for all the workloads, achieving at least 1.2$\times$ higher average data-reduction ratios.
%Second, \prop significantly outperforms Finesse in most workloads.
\js{First,} \prop significantly outperforms Finesse in most workloads.
Except for \pc{} in which \prop provides the similar data-reduction ratio with Finesse, \prop exhibits up to 33\% (on average 21\%) higher data-reduction ratios than Finesse. 
%Fourth, \prop significantly outperforms both SFSketch and Finesse under \sof{} workloads, achieving \emph{at least} 24.4\% data reduction improvement.
In particular, \prop greatly improves the data-reduction ratio by \emph{at least} 24\% over Finesse under \sof{} workloads.
This suggests that 1) \prop can improve the data-reduction efficiency for workloads that the state-of-the-art SF-based search technique cannot effectively cope with, and 2) \prop has high adaptability (\ie~it can work efficiently for data sets that are not used for the DNN training).
Second, \prop provides higher data-reduction ratios even for highly compressible workloads.
Under \web, Finesse significantly reduces the write traffic by about 80\% over noDC, but \prop increases the data-reduction ratio even further by 33\% compared to Finesse.  
%From our observations, we conclude that \prop is an effective solution to maximize the data-reduction ratio of post-deduplication delta compression for various workloads.
From our observations, we conclude that \prop is an effective solution to maximize the data-reduction ratio for various workloads.

\vspace{-1em}
\subsection{Reference Search Pattern Analysis\label{subsec:pattern}}
\vspace{-.5em}
To better understand how \prop can outperform the state-of-the-art technique, we analyze the reference-search efficiency of \prop and Finesse.
%To better understand how \prop can outperform the state-of-the-art reference search technique in detail, we analyze the reference-search efficiency of \prop and Finesse.
Given a data block $B$, we measure $S_{FS}(B)$ and $S_{DS}(B)$, the number of \emph{saved bytes} by Finesse and \prop, respectively.
$S_{FS}(B)$ (or $S_{DS}(B)$) is obtained by subtracting the size of $B$ when delta-compressed with the reference block found by Finesse (or \prop) from the original size of $B$ (\ie~4 KiB).
%$S_{FS}(B)$ (or $S_{DS}(B)$) is obtained by subtracting the size of $B$ when delta-compressed with the reference block suggested by Finesse (or \prop) from the original size of $B$ (\ie~4 KiB).
The larger the $S_{FS}(B)$ (or $S_{DS}(B)$) value, the higher the reference-search efficiency. 
If a reference search technique fails to find a reference block for $B$, we compress it using the LZ4 algorithm and then use the compressed size to calculate data saving.

\fig{\ref{fig:pattern}} plots coordinates of $x=$~$S_{FS}(B_i)$ and $y=$~$S_{DS}(B_i)$ for a block $B_i$ in each workload.
If $x = y$, Finesse and \prop exhibit the same delta-compression ratio (highlighted with a red line in \fig{\ref{fig:pattern}}), which implies that they select the same reference block. 
%If $x = y$ (\ie~$S_{FS}(B_i)$ $=$ $S_{DS}(B_i)$), Finesse and \prop exhibit the same delta-compression ratio (highlighted with a red line in \fig{\ref{fig:pattern}}), which implies that they select the same reference block.
A coordinate ($S_{FS}(B_i)$, $S_{DS}(B_i)$) above (or below) the line means that \prop provides higher (or lower) data-reduction ratio for block $B_i$ than Finesse.
%If a coordinate ($S_{FS}(B_i)$, $S_{DS}(B_i)$) is plotted above (or below) the line, it means that \prop provides higher (or lower) compression ratio for block $B_i$ than Finesse.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/r_pattern.pdf}
    \vspace{-2em}
    \caption{Comparison of the reference-search pattern.}
    \label{fig:pattern}
    \vspace{-1.5em}
\end{figure}

From \fig{\ref{fig:pattern}}, we make three observations.  
First, as expected, \prop provides higher data savings compared to Finesse for a large number of blocks under every workload. %except for \pc{}.  
% \fix{In \fig{\ref{fig:pattern}(a)} from \pc{}, the coordinates ($S_{FS}(B_i)$, $S_{DS}(B_i)$) are distributed almost evenly in regions where $y > x$ and $ y < x$.}
% Therefore, \prop and Finesse exhibit almost the same data reduction under \pc{}. 
Second, despite the higher data savings of \prop over Finesse in general, there are also a non-trivial number of blocks for which Finesse selects better references, achieving higher data savings than \prop.  
Excluding the \sof{} workloads, Finesse selects higher-quality references compared to \prop for up to 11.8\% of the total blocks.
Third, \prop and Finesse show quite different patterns in reference search.
As shown in \fig{\ref{fig:pattern}}, the coordinates in $y > x$ region (\ie~where \prop outperforms Finesse) are close to the line $y = x$, and at the same time, many of them are scattered across a wide range of the region compared to the coordinates in $y < x$ region.
On the other hand, a majority of the coordinates in $y < x$ region (\ie~where Finesse outperforms \prop) tend to have a very large $y$ value (\eg~> 3,072).
These imply that, while Finesse is effective to find a reference highly similar to an input block, it also misses a number of blocks that \prop can find and use to improve the data-reduction efficiency. 

\vspace{-1em}
\subsection{Combination with Existing Techniques\label{subsec:combined}}
\vspace{-.5em}
Our second and third observations in \sect{\ref{subsec:pattern}} motivate us to combine \prop with existing techniques to maximize the data-reduction ratio.
%Our second and third observations in \sect{\ref{subsec:pattern}} motivate us to combine \prop with existing reference search techniques to maximize the data-reduction ratio.
We design a storage system that employs both Finesse and \prop.  
When the two techniques find different reference blocks for an incoming block, the system chooses the one that provides a higher data-reduction ratio.
%When the two reference search techniques find different reference blocks for an incoming block, the system chooses the one that provides a higher data-reduction ratio.
Such an approach increases the memory and computation overheads for data sketching but would be desirable for a system where data reduction is paramount (\eg~backup systems).
%Although such an approach increases the memory and computation overheads for data sketching, it would be desirable for a system where data reduction is the highest priority (\eg~backup systems).
We leave the study of efficiently combining \prop with existing techniques as future work.

\fig{\ref{fig:combined}} shows the combined approach's data-reduction benefits compared to when using either Finesse or \prop{} alone.\footnote{
%\fig{\ref{fig:combined}} shows how much the combined approach can improve the data-reduction ratio compared to when using either Finesse or \prop{} alone.\footnote{
We omit the results of the \sof{} workloads in \fig{\ref{fig:combined}} because there is no motivation to combine \prop{} with Finesse under such workloads for which Finesse provides negligible data reduction.} 
We also measure the \emph{optimal} data-reduction ratio (\ie~when every data block is delta-compressed with the best reference block found by brute-force search) for each workload to understand room for improvement after applying the combined approach.  
To emphasize the benefits of the combined approach over the standalone techniques, we normalize all the results in \fig{\ref{fig:combined}} to Finesse.
%To emphasize the benefits of the combined approach over the standalone reference search techniques, we normalize all the results in \fig{\ref{fig:combined}} to Finesse.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/r_combined.pdf}
    \vspace{-1.5em}
    \caption{Data-reduction improvement of a combination of \prop and Finesse.}
    \label{fig:combined}
    \vspace{-1.5em}
\end{figure}

We observe that, as expected, the combined approach further improves the data-reduction ratio compared to the two standalone techniques under most workloads.
%We observe that, as expected, the combined approach further improves the data-reduction ratio compared to the two standalone reference search techniques under most workloads.
The combined approach achieves up to 38\% and 6.6\% (15\% and 4.8\% on average) data-reduction improvements over Finesse and \prop, respectively.
%The combined approach achieves up to 38\% and 6.6\% (15\% and 4.8\% on average) improvements in data-reduction ratio over Finesse and \prop, respectively.
We also observe that the combined approach can reduce the gap in data-reduction ratios between the existing reference search techniques and the optimal.  
Although there is still large room for improvement (\ie~up to 35\% and 26\% on average) even after applying the combined approach, the combined approach reduces the gap by up to 81\% (\ie~62\% $\rightarrow$ 9.6\% under \web) and by 42\% on average. 
From our observations, we conclude that \prop can also be used as a useful method
to complement the weakness of existing post-deduplication delta compression techniques.

%JS: I think this subsection is the best candidate to be removed.
\vspace{-1em}
\subsection{Multi-candidate \prop\label{subsec:multi}}
\vspace{-.5em}
We explore the possibility of reducing write traffic by considering multiple candidates when choosing a reference block.
%We explore the possibility of reducing write traffic by taking into account multiple candidates when choosing a reference block.  
%Our storage platform adopts the first-fit selection approach by default. 
%For example, Finesse chooses the first matching block as a reference even though there exist many candidates. 
%Similarly, the ANN engine of \prop returns only a single reference, which is considered the most similar to an incoming block, among many candidates. 
As explained in \sects{\ref{subsec:motiv_lsh} and \ref{subsec:select}}, both \prop and SF-based techniques are able to consider multiple reference blocks in choosing a reference by design.
%However, as explained in \sects{\ref{subsec:motiv_lsh} and \ref{subsec:select}}, both \prop and SF-based techniques are able to consider multiple reference blocks in choosing a reference by design.
This gives us a great potential to increase the data-reduction ratio by looking up many candidates and choosing the best one.
Doing so might incur additional computation and I/O costs, but it would not be a serious obstacle if data reduction is the highest priority.  

To evaluate the impact of the multi-candidate approach on data-reduction efficiency, we measure the write traffic, \ie~the amount of data physically written to the storage system, while increasing the number $N_{C}$ of candidates to 20, as shown in \fig{\ref{fig:multi}} (all the results are normalized to noDC).
Instead of using the first-fit reference, our system is enhanced to retrieve top-$N_{C}$ candidates from the SK store (in Finesse) or from the ANN engine (in \prop). 
The storage system then performs delta compression for each candidate and finally chooses one that exhibits the highest compression ratio.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/r_multi.pdf}
    \vspace{-1.5em}
    \caption{Effect of using multiple reference candidates.}
    \vspace{-1.5em}
    \label{fig:multi}
\end{figure}

We make two observations from our results.
First, the benefits of using multiple reference candidates significant varies across workloads.
%First, the benefits of using multiple reference candidates are highly dependent upon characteristics of workloads.  
For \synth, \sensor, and \web, increasing $N_C$ to 20 allows \prop{} to further reduce the write traffic considerably by 6.58\%, 10.9\%, and 9.1\%, respectively, compared to when $N_C = 1$.
In contrast, for the remaining workloads, no huge benefits are observed.
Second, unlike \prop, Finesse does not show meaningful write-traffic reduction with multiple candidates except for \web.
%Second, unlike \prop, Finesse fails to bring a meaningful reduction in the write traffic with multiple candidates except for \web. 
According to our analysis, different reference candidates found by Finesse provide similar delta-compression ratios for the same incoming block.
This can be explained with the way of generating SF-based sketches in Finesse.
%This can be explained with the way of extracting the hash values (\ie~features) from a block and of building a super feature (SF) in Finesse.  
Even though two different blocks could have one or more identical SFs, its probability drastically decreases as the difference between the two blocks increases.
Such a characteristic allows Finesse to find only highly similar references to an incoming block, which leads to little variations in the similarity within multiple reference candidates found by Finesse.  
In contrast, \prop{} does not rely on hashing to generate a sketch and thus gives us opportunities to find a more suitable reference among candidates.

\begin{figure}[!b]
    \centering
    \vspace{-1em}
    \includegraphics[width=0.75\linewidth]{figs/r_training}
    \vspace{-.5em}
    \caption{Effect of the training data-set size.}
    %\caption{Impact of the training data-set size on the data-reduction ratio of \prop.}
    \label{fig:tdata}
\end{figure}


\vspace{-1em}
\subsection{Impact of the Training Data-Set Size\label{subsec:tdata}}
\vspace{-.5em}
We evaluate the impact of the training data-set size on the data-reduction ratio of \prop.
\fig{\ref{fig:tdata}} shows the average data-reduction ratio of \prop for entire workloads while we change the fraction of each trace used for training \prop's DNN model from 1\% to 10\%.
When we use $x$\% ($<$ 10\%) of each trace for training, we use the remaining $(100-x)$\% to evaluate the data-reduction ratio of \prop.
All values in \fig{\ref{fig:tdata}} are normalized to the data-reduction ratio when the fraction of training data is 10\%.

We observe that the larger the training data set, the higher the data-reduction ratio that \prop achieves.
%As shown in \fig{\ref{fig:tdata}}, the larger the training data set, the higher the data-reduction ratio that \prop achieves.
However, \prop also can provide a fairly good data-reduction ratio even with a very small training data set: using only 1\% of the traces for DNN training provides 98.9\% of the data-reduction ratio when we use 10\% of the traces.  
We conclude that we can maximize the data-reduction ratio of \prop by increasing the size of the training data set, but we can also provide a sufficiently high data-reduction ratio with a small amount of DNN training time even for large data sets.

%JS: If we include the throughput results, overhead analysis becomes 1 page. Does it make sense to discuss it this much?
\vspace{-1em}
\subsection{Overhead Analysis\label{subsec:overhead}}
\vspace{-.5em}
\head{Performance Overhead}
\fig{\ref{fig:throughput}} shows the average throughput of \prop and the combined approach of \prop and Finesse under different workloads, normalized to Finesse.
\prop and combined approach provide up to 73.7\% and 44.9\% (44.6\% and 28.4\% on average across all workloads) of the average throughput of Finesse.
This non-trivial performance overhead is due to the inherent trade-off between the data-reduction ratio and throughput in post-deduplication delta compression; performing delta compression for more data blocks would increase the data reduction ratio, but it comes at the cost of performance degradation since delta compression takes more time compared to lossless compression (\eg~in our current implementation, LZ4 takes 6.9~\usec per block on average, which is less than 10\% of the average execution time of Xdelta).
% \fix{
% We also compare the system throughput of \prop and SFSketch.
% \fig{\ref{fig:throughput}} shows the average throughput of \prop under different workloads, normalized to SFSketch.
% \prop provides up to 74.9\% (24.9\% on average across all workloads) of the average throughput of SKSketch, showing higher performance overhead than our expectation with the latency analysis above.
% This is due to the inherent trade-off between the data reduction ratio and throughput in post-deduplication delta compression: performing delta compression for more data blocks would increase the data reduction ratio, but it comes at the cost of performance degradation since delta compression takes more time compared to lossless compression (\eg~in our current implementation, LZ4 takes 6.9~\usec per block on average, which is less than 10\% of the average execution time of Xdelta).

\begin{figure}[!h]
    \centering
    \vspace{-.5em}
    \includegraphics[width=\linewidth]{figs/throughput.pdf}
    \vspace{-1.5em}
    \caption{Performance overheads of \prop.}
    \vspace{-.5em}
    \label{fig:throughput}
\end{figure}

To better understand the performance overheads of \prop, we measure the average latency of each step per input data block during the post-deduplication delta compression process.
\prop requires two modifications on existing techniques, 1) replacing the SF-based sketching engine with the DNN-based one and 2) using the ANN engine described in \sect{\ref{subsec:select}} as the SK store.
For fair comparison, we implement the SK store of Finesse using the unordered-map data structure that provides $O(1)$ time complexity for lookup.
\fig{\ref{fig:overhead}} visualizes the fraction of the average time spent for each step in the entire data reduction process. 

As shown in \fig{\ref{fig:overhead}}, \prop and Finesse operate differently in only three steps of the entire data reduction process: 1) sketch generation for an incoming block, 2) sketch retrieval from the SK store, and 3) sketch update to the SK store.
The other steps, including deduplication, Xdelta compression, and LZ4 compression, are performed in the same ways. 
Due to the simplicity of the hash network model network and GPU acceleration, \prop reduces the latency of sketch generation from 88.73 \usec to 36.47 \usec (by 58.9\%) over Finesse.
However, using the ANN engine significantly increases the latencies for sketch retrieval and update, leading to 55.1\% increase in the total average latency over Finesse. 
%However, the ANN engine executed by CPUs increases the latencies for sketch retrieval and update significantly, which, in turn, leads to 55.1\% increase in the average latency for data reduction over Finesse.   

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/r_overhead.pdf}
    \vspace{-2em}
    \caption{Average latency for each data reduction step in (a) DeepSketch and (b) Finesse.}
    \vspace{-1.5em}
    \label{fig:overhead}
\end{figure}

The performance overhead of \prop is non-trivial, but it would not be a serious obstacle for its wide adoption due to two reasons.
%The additional performance overhead of \prop is non-trivial, but it would not be a serious obstacle for its wide adoption.
First, we target a system where data reduction is critically important so that \prop's benefits outweigh its performance overheads.
%First, post-deduplication delta compression is typically used in a system where the data-reduction efficiency is more important than performance.
%Considering the data reduction process is performed in \emph{background}, its negative impact on user-perceived performance would be relatively small.
Second, the performance overhead of \prop can be mitigated in several ways.
For example, if the data reduction process is performed in \emph{background}, its negative performance impact could be relatively small.
%The current ANN engine is designed to run on CPUs.
%By improving it to use ML accelerators (\eg~GPU, FPGA, or NPU), we can reduce sketch update and retrieval times.
We can also leverage the parallelism of multi-core CPUs to optimize software modules.
%We can also leverage the parallelism of multi-core CPUs to optimize software modules that are not easily accelerated by ML accelerators.
For example, the sketch update procedure can be performed in parallel with other modules. 
This hides the cost of updating sketches during the compression steps, thereby reducing the performance overhead by 45.8\% (\ie~103.98 \usec $\rightarrow$ 56.27 \usec).

\head{Memory Overhead}
Like existing post-deduplication delta compression techniques~\cite{shilane-fast-2012, zhang-fast-2019}, \prop inevitably requires additional memory space for the sketch store. 
%The memory space required by the sketch store is proportional to 1) the sketch size and 2) the number of sketches kept in the sketch store.
Despite the smaller sketch size of \prop compared to existing techniques~\cite{shilane-fast-2012, zhang-fast-2019} (128 bits vs. 192 bits), \prop's memory overhead might be unacceptable if it keeps track of the sketches of \emph{all} non-deduplicated data blocks.
For example, suppose that the data block size is 4 KiB, and 80\% of the stored data is unique (\ie~non-deduplicated). 
Then, the required memory space for the sketch store is about 0.3\% (0.8$\times$16/4,096) of the size of the stored data (e.g., around 100-GB memory space to work with 32-TB data).
%Then, the required memory space for the sketch store is about 0.3\% (0.8$\times$16/4,096) of the size of the stored data, which means that \prop requires at least 100-GB memory space to work with 32-TB data. 

However, the memory overhead would not be a significant obstacle \sj{to use \prop in practice for two reasons}.
First, the memory overhead for the sketch store is a common problem in \sj{all the sketch-based techniques}. 
Second, prior works demonstrate that a small fraction of data blocks are frequently used as the reference block for many input blocks~\cite{gupta-fast-2011, park-date-2017}.
Thus, keeping only least-frequently-used (LFU) sketches in a limited-size sketch store would provide sufficiently high compression efficiency.
We leave such further optimizations to mitigate \prop's memory overhead for future work. 

